Variational Inference via $\chi$-Upper Bound Minimization

Variational inference (VI) is widely used as an efficient alternative to Markov chain Monte Carlo. It posits a family of approximating distributions $q$ and finds the closest member to the exact posterior $p$. Closeness is usually measured via a divergence $D(q || p)$ from $q$ to $p$. While successful, this approach also has problems. Notably, it typically leads to underestimation of the posterior variance. In this paper we propose CHIVI, a black-box variational inference algorithm that minimizes $D_{\chi}(p || q)$, the $\chi$-divergence from $p$ to $q$. CHIVI minimizes an upper bound of the model evidence, which we term the $\chi$ upper bound (CUBO). Minimizing the CUBO leads to improved posterior uncertainty, and it can also be used with the classical VI lower bound (ELBO) to provide a sandwich estimate of the model evidence. We study CHIVI on three models: probit regression, Gaussian process classification, and a Cox process model of basketball plays. When compared to expectation propagation and classical VI, CHIVI produces better error rates and more accurate estimates of posterior variance.

==> preamble/preamble.tex <==
% # FONTS

\usepackage[T1]{fontenc}
\usepackage{tgtermes}

% NOTE: MUST INSTALL SEPARATELY
% \usepackage[subscriptcorrection,
%            amssymbols,
%            mtpbb,
%            mtpcal,
%            nofontinfo  % suppresses all warnings
%           ]{mtpro2}
% NOTE: MUST UNCOMMENT IF NOT USING MTPRO2
\usepackage{amssymb}
\newcommand{\mathbold}[1]{\ensuremath{\boldsymbol{\mathbf{#1}}}}

\usepackage{scalefnt,letltxmacro}
\LetLtxMacro{\oldtextsc}{\textsc}
\renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.10}#1}}
% \renewcommand*\ttdefault{lmvtt}
\usepackage[ttdefault=true]{AnonymousPro}

% # MATH

\usepackage{amsmath}

% # SPACING and TEXT
usepackage[
  paper  = letterpaper,
   %left   = 1.25in,
   textwidth=5.5in,
    textheight=9in,
    headheight=12pt,
    headsep=25pt,
    footskip=30pt,
   %right  = 1.25in,
   top    = 1.0in,
   bottom = 1.0in,
   ]{geometry}
   
% \usepackage[final,expansion=alltext]{microtype}
\usepackage[english]{babel}
\usepackage[parfill]{parskip}
\usepackage{afterpage}
\usepackage{enumitem}
\usepackage{framed}
\usepackage{xspace}

% # EDITING

\usepackage{lineno}
\renewcommand\linenumberfont{\normalfont
                             \footnotesize
                             \sffamily
                             \color{SkyBlue}}

\usepackage{ragged2e}
\DeclareRobustCommand{\sidenote}[1]{\marginpar{
                                    \RaggedRight
                                    \textcolor{Plum}{\textsf{#1}}}}

\newcommand{\parnum}{\bfseries\P\arabic{parcount}}
\newcounter{parcount}
\newcommand\p{%
    \stepcounter{parcount}%
    \leavevmode\marginpar[\hfill\parnum]{\parnum}%
}
\DeclareRobustCommand{\parhead}[1]{\textbf{#1}~}
\setlength{\marginparwidth}{0.5in} % For sidenotes on two-column papers

% # COLOR

\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{shadecolor}{gray}{0.9}

\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\sky}[1]{\textcolor{SkyBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}

% # COUNTERS

\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% # FIGURES

\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
\usepackage[format=hang]{subcaption}

% # TABLES

\usepackage{booktabs, array}

% # ALGORITHMS

\usepackage[algoruled]{algorithm2e}
\setlength{\interspacetitleruled}{8pt}
\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\small}

% # BIBLIOGRAPHY AND LINKS

\usepackage{natbib}
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=MidnightBlue}
\hypersetup{linkcolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}
\usepackage[nameinlink]{cleveref}
\creflabelformat{equation}{#2\textup{#1}#3}  % <- remove parenthesis from equations

% # ACRONYMS

\usepackage
[acronym,smallcaps,nowarn,section,nogroupskip,nonumberlist]{glossaries}
\glsdisablehyper{}

% # CODE SNIPPETS

\lstdefinestyle{mystyle}{
    commentstyle=\color{OliveGreen},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{BrickRed},
    basicstyle=\ttfamily\scriptsize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=none,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle}

% # USEFUL COMMANDS

\newcommand{\pp}{\textcolor{Plum}{\P\,}}
\newcommand{\q}[1]{\red{{\sf Q | #1}}}
\newcommand{\draftdisclaimer}{\begin{center}\begin{framed} DRAFT: DO
NOT CITE OR DISTRIBUTE \end{framed}\end{center}}


==> preamble/preamble_acronyms.tex <==
\newacronym{CUBO}{cubo}{$\chi$ upper bound}
\newacronym{BBVI}{bbvi}{black box variational inference}
\newacronym{ELBO}{elbo}{evidence lower bound}
\newacronym{EP}{ep}{expectation propagation}
\newacronym{GP}{gp}{Gaussian process}
\newacronym{VI}{vi}{Variational inference}
\newacronym{KL}{kl}{Kullback-Leibler}
\newacronym{MCMC}{mcmc}{Markov chain Monte Carlo}
\newacronym{HMC}{hmc}{Hamiltonian Monte Carlo}
\newacronym{chiVI}{chivi}{$\chi$-divergence variational inference}
\newacronym{klVI}{klvi}{$\operatorname{KL}(q || p)$ variational inference}


==> preamble/preamble_math.tex <==
% # PROBABILITY

\newcommand{\g}{\,|\,}
\renewcommand{\gg}{\,\|\,}
\DeclareRobustCommand{\KL}[2]{\ensuremath{\textrm{KL}\left(#1\;\|\;#2\right)}}
\newcommand{\ind}{\mathbb{1}}

% # DISTRIBUTIONS

\newcommand{\Gam}{\textrm{Gam}}
\newcommand{\InvGam}{\textrm{InvGam}}

% # MISCELLANEOUS

\renewcommand{\d}[1]{\ensuremath{\operatorname{d}\!{#1}}}
\newcommand{\diag}{\textrm{diag}}
\newcommand{\supp}{\textrm{supp}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\E}[1]{\mathbb{E}\left[ #1 \right]}
\newcommand{\EE}[2]{\mathbb{E}_{#1}\left[ #2 \right]}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\rep}{\textrm{rep}}

\newtheorem{theorem}{Theorem}
\newtheorem{thm}{Theorem} 

% # BOLD MATHEMATICS

\newcommand{\mba}{\mathbold{a}}
\newcommand{\mbb}{\mathbold{b}}
\newcommand{\mbc}{\mathbold{c}}
\newcommand{\mbd}{\mathbold{d}}
\newcommand{\mbe}{\mathbold{e}}
%\newcommand{\mbf}{\mathbold{f}}
\newcommand{\f}{\mathbold{f}}
\newcommand{\mbg}{\mathbold{g}}
\newcommand{\mbh}{\mathbold{h}}
\newcommand{\mbi}{\mathbold{i}}
\newcommand{\mbj}{\mathbold{j}}
\newcommand{\mbk}{\mathbold{k}}
\newcommand{\mbl}{\mathbold{l}}
\newcommand{\mbm}{\mathbold{m}}
\newcommand{\mbn}{\mathbold{n}}
\newcommand{\mbo}{\mathbold{o}}
\newcommand{\mbp}{\mathbold{p}}
\newcommand{\mbq}{\mathbold{q}}
\newcommand{\mbr}{\mathbold{r}}
\newcommand{\mbs}{\mathbold{s}}
\newcommand{\mbt}{\mathbold{t}}
\newcommand{\mbu}{\mathbold{u}}
\newcommand{\mbv}{\mathbold{v}}
\newcommand{\mbw}{\mathbold{w}}
\newcommand{\mbx}{\mathbold{x}}
\newcommand{\mby}{\mathbold{y}}
\newcommand{\mbz}{\mathbold{z}}

\newcommand{\mbA}{\mathbold{A}}
\newcommand{\mbB}{\mathbold{B}}
\newcommand{\mbC}{\mathbold{C}}
\newcommand{\mbD}{\mathbold{D}}
\newcommand{\mbE}{\mathbold{E}}
\newcommand{\mbF}{\mathbold{F}}
\newcommand{\mbG}{\mathbold{G}}
\newcommand{\mbH}{\mathbold{H}}
\newcommand{\mbI}{\mathbold{I}}
\newcommand{\mbJ}{\mathbold{J}}
\newcommand{\mbK}{\mathbold{K}}
\newcommand{\mbL}{\mathbold{L}}
\newcommand{\mbM}{\mathbold{M}}
\newcommand{\mbN}{\mathbold{N}}
\newcommand{\mbO}{\mathbold{O}}
\newcommand{\mbP}{\mathbold{P}}
\newcommand{\mbQ}{\mathbold{Q}}
\newcommand{\mbR}{\mathbold{R}}
\newcommand{\mbS}{\mathbold{S}}
\newcommand{\mbT}{\mathbold{T}}
\newcommand{\mbU}{\mathbold{U}}
\newcommand{\mbV}{\mathbold{V}}
\newcommand{\mbW}{\mathbold{W}}
\newcommand{\mbX}{\mathbold{X}}
\newcommand{\mbY}{\mathbold{Y}}
\newcommand{\mbZ}{\mathbold{Z}}

\newcommand{\mbalpha}{\mathbold{\alpha}}
\newcommand{\mbbeta}{\mathbold{\beta}}
\newcommand{\mbdelta}{\mathbold{\delta}}
\newcommand{\mbepsilon}{\mathbold{\epsilon}}
\newcommand{\mbchi}{\mathbold{\chi}}
\newcommand{\mbeta}{\mathbold{\eta}}
\newcommand{\mbgamma}{\mathbold{\gamma}}
\newcommand{\mbiota}{\mathbold{\iota}}
\newcommand{\mbkappa}{\mathbold{\kappa}}
\newcommand{\mblambda}{\mathbold{\lambda}}
\newcommand{\mbmu}{\mathbold{\mu}}
\newcommand{\mbnu}{\mathbold{\nu}}
\newcommand{\mbomega}{\mathbold{\omega}}
\newcommand{\mbphi}{\mathbold{\phi}}
\newcommand{\mbpi}{\mathbold{\pi}}
\newcommand{\mbpsi}{\mathbold{\psi}}
\newcommand{\mbrho}{\mathbold{\rho}}
\newcommand{\mbsigma}{\mathbold{\sigma}}
\newcommand{\mbtau}{\mathbold{\tau}}
\newcommand{\mbtheta}{\mathbold{\theta}}
\newcommand{\mbupsilon}{\mathbold{\upsilon}}
\newcommand{\mbvarepsilon}{\mathbold{\varepsilon}}
\newcommand{\mbvarphi}{\mathbold{\varphi}}
\newcommand{\mbvartheta}{\mathbold{\vartheta}}
\newcommand{\mbvarrho}{\mathbold{\varrho}}
\newcommand{\mbxi}{\mathbold{\xi}}
\newcommand{\mbzeta}{\mathbold{\zeta}}

\newcommand{\mbDelta}{\mathbold{\Delta}}
\newcommand{\mbGamma}{\mathbold{\Gamma}}
\newcommand{\mbLambda}{\mathbold{\Lambda}}
\newcommand{\mbOmega}{\mathbold{\Omega}}
\newcommand{\mbPhi}{\mathbold{\Phi}}
\newcommand{\mbPi}{\mathbold{\Pi}}
\newcommand{\mbPsi}{\mathbold{\Psi}}
\newcommand{\mbSigma}{\mathbold{\Sigma}}
\newcommand{\mbTheta}{\mathbold{\Theta}}
\newcommand{\mbUpsilon}{\mathbold{\Upsilon}}
\newcommand{\mbXi}{\mathbold{\Xi}}

\newcommand{\mbzero}{\mathbold{0}}
\newcommand{\mbone}{\mathbold{1}}
\newcommand{\mbtwo}{\mathbold{2}}
\newcommand{\mbthree}{\mathbold{3}}
\newcommand{\mbfour}{\mathbold{4}}
\newcommand{\mbfive}{\mathbold{5}}
\newcommand{\mbsix}{\mathbold{6}}
\newcommand{\mbseven}{\mathbold{7}}
\newcommand{\mbeight}{\mathbold{8}}
\newcommand{\mbnine}{\mathbold{9}}

